User-Driven Functional Movement Training with a Wearable Hand Robot after Stroke

We studied the performance of a robotic orthosis designed to assist the paretic hand after stroke. It is wearable and fully user-controlled, serving two possible roles: as a therapeutic tool that facilitates device mediated hand exercises to recover neuromuscular function or as an assistive device for use in everyday activities to aid functional use of the hand. We present the clinical outcomes of a pilot study designed as a feasibility test for these hypotheses. 11 chronic stroke (> 2 years) patients with moderate muscle tone (Modified Ashworth Scale less than or equal to 2 in upper extremity) engaged in a month-long training protocol using the orthosis. Individuals were evaluated using standardized outcome measures, both with and without orthosis assistance. Fugl-Meyer post intervention scores without robotic assistance showed improvement focused specifically at the distal joints of the upper limb, suggesting the use of the orthosis as a rehabilitative device for the hand. Action Research Arm Test scores post intervention with robotic assistance showed that the device may serve an assistive role in grasping tasks. These results highlight the potential for wearable and user-driven robotic hand orthoses to extend the use and training of the affected upper limb after stroke.

==> Makefile <==
DIR := $(shell pwd)
PAPER := journal2019_orthosis

paper:
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \
	bibtex pdf/$(PAPER).aux; \
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \
	pdflatex -output-directory pdf --jobname=$(PAPER) ms.tex; \

clean:
	rm -f pdf/*; \
	rm -f *.bbl; \
	rm -f $(PAPER)_arxiv.tgz; \

arxiv: paper
	rm -f $(PAPER)_arxiv.tgz; \
	touch $(PAPER)_arxiv.tgz; \
	cp pdf/$(PAPER).bbl ./ms.bbl; \
	tar --exclude=$(PAPER)_arxiv.tgz -cvzf $(PAPER)_arxiv.tgz --exclude-vcs --exclude=extra --exclude=download --exclude=bib --exclude=pdf --exclude=Makefile --exclude=*~ .

all: paper

